Hyperparameter Optimization for SecureBoost via Constrained Multi-Objective Federated Learning

SecureBoost is a tree-boosting algorithm that leverages homomorphic encryption (HE) to protect data privacy in vertical federated learning. SecureBoost and its variants have been widely adopted in fields such as finance and healthcare. However, the hyperparameters of SecureBoost are typically configured heuristically for optimizing model performance (i.e., utility) solely, assuming that privacy is secured. Our study found that SecureBoost and some of its variants are still vulnerable to label leakage. This vulnerability may lead the current heuristic hyperparameter configuration of SecureBoost to a suboptimal trade-off between utility, privacy, and efficiency, which are pivotal elements toward a trustworthy federated learning system. To address this issue, we propose the Constrained Multi-Objective SecureBoost (CMOSB) algorithm, which aims to approximate Pareto optimal solutions that each solution is a set of hyperparameters achieving an optimal trade-off between utility loss, training cost, and privacy leakage. We design measurements of the three objectives, including a novel label inference attack named instance clustering attack (ICA) to measure the privacy leakage of SecureBoost. Additionally, we provide two countermeasures against ICA. The experimental results demonstrate that the CMOSB yields superior hyperparameters over those optimized by grid search and Bayesian optimization regarding the trade-off between utility loss, training cost, and privacy leakage.

==> sections/0_abstract.tex <==
% SecureBoost is a tree-boosting algorithm leveraging homomorphic encryption to protect data privacy in the vertical federated learning setting. It is widely used in fields such as finance and healthcare due to its interpretability, effectiveness, and privacy-preserving capability. However, SecureBoost suffers from high computational complexity and risk of label leakage. To harness the full potential of SecureBoost, hyperparameters of SecureBoost should be carefully chosen to strike an optimal balance between utility, efficiency, and privacy. Existing methods either set hyperparameters empirically or heuristically, which are far from optimal. To fill this gap, we propose a Constrained Multi-Objective SecureBoost (CMOSB) algorithm to find Pareto optimal solutions that each solution is a set of hyperparameters achieving optimal tradeoff between utility loss, training cost, and privacy leakage. We design measurements of the three objectives. \red{In particular, the privacy leakage is measured using our proposed instance clustering attack. Experimental results demonstrate that the CMOSB yields not only hyperparameters superior to the baseline but also optimal sets of hyperparameters that can support the flexible requirements of FL participants. }

SecureBoost is a tree-boosting algorithm leveraging homomorphic encryption to protect data privacy in vertical federated learning. It is widely used in fields such as finance and healthcare due to its interpretability and generality. However, SecureBoost suffers from high computational complexity and risk of label leakage. To harness the full potential of SecureBoost, hyperparameters of SecureBoost should be carefully chosen to strike an optimal balance between utility, efficiency, and privacy. Existing methods either set hyperparameters empirically or heuristically, which are far from optimal. To fill this gap, we propose a Constrained Multi-Objective SecureBoost (CMOSB) algorithm aiming to approximate Pareto fronts, in which each solution is a set of hyperparameters achieving optimal tradeoff between utility loss, training cost, and privacy leakage. We design measurements of the three objectives. In particular, we develop an instance clustering attack (ICA) as a way to measure the privacy leakage of SecureBoost and propose two countermeasures against ICA. Experimental results demonstrate that the CMOSB yields superior hyperparameters over those optimized by grid search and Bayesian optimization in terms of the tradeoff between utility loss, training cost, and privacy leakage. 
% Moreover, CMOSB can find Pareto optimal solutions of hyperparameters that achieve the optimal tradeoffs between utility loss, training cost, and privacy leakage.


==> sections/1_intro_backup.tex <==
\section{Introduction}

Federated learning~\cite{DBLP:conf/aistats/McMahanMRHA17,DBLP:journals/debu/TongZZLSL0L23} is a novel distributed machine learning paradigm that enables multiple participants to train machine learning models using participants' private data without compromising data privacy. 
% joint modeling and learning by transmitting only gradients or intermediate results, effectively preserving privacy. 
SecureBoost~\cite{DBLP:journals/expert/ChengFJLCPY21} is a widely-used vertical federated tree-boosting algorithm for its interpretability and effectiveness. It has been widely applied in many fields, such as advertisement\cite{Yang2020}, finance\cite{yang2019federated,9671857}, and healthcare\cite{DBLP:journals/jhir/XuGSWBW21}. 
% For instance, banks can use it to jointly predict customers' credit ratings by utilizing e-commerce data. 

% To protect data privacy, SecureBoost applies homomorphic encryption ~\cite{DBLP:conf/eurocrypt/Paillier99} to the gradient of training samples. However, the efficiency of homomorphic encryption is too low, which leads to huge time costs when dealing with large-scale data, which is unacceptable to some extent. The homomorphic encryption only protects a portion of the intermediate results, and some studies~\cite{DBLP:conf/icde/LuoWXO21} have shown that there is still a possibility of data leakage in vertically federated learning. SecureBoost, due to the lack of protection for sample distribution, may also result in label leakage. 

SecureBoost applies \textit{homomorphic encryption} (HE)~\cite{DBLP:conf/eurocrypt/Paillier99} to protect data privacy. 
However, HE is computationally expensive, which hinders SecureBoost from being applied to large-scale machine learning problems. 
% However, HE is computationally expensive, which hinders SecureBoost from being applied in large-scale data federation~\cite{DBLP:journals/pvldb/TongPZSXZZCXXL22}. 
% low, which leads to huge time costs when dealing with large-scale data, which is unacceptable to some extent. 
In addition, we demonstrate that SecureBoost suffers from the instance clustering attack (ICA), a label inference attack that we propose to infer labels of the active party. In other words, SecureBoost has the risk of leaking labels (see Sec. \ref{sec:priv}). We design two countermeasures against ICA but at the expense of losing utility.
% The homomorphic encryption only protects a portion of the intermediate results, and some studies~\cite{DBLP:conf/icde/LuoWXO21} have shown that there is still a possibility of data leakage in vertically federated learning. SecureBoost, due to the lack of protection for sample distribution, may also result in label leakage. 

To harness the full potential of SecureBoost, its hyperparameters (including hyperparameters of the applied protection mechanism) should be set such that the utility loss, training cost, and privacy leakage can be minimized simultaneously, and the optimal tradeoffs between utility, efficiency, and privacy can be achieved. However, existing FL platforms~\cite{DBLP:journals/jmlr/LiuFCXY21,DBLP:conf/sigmod/FuSYJXT021} often set the hyperparameters of SecureBoost to empirical values or apply heuristic methods to search for the hyperparameters to tradeoff between utility, efficiency, and privacy. These existing methods may lead to hyperparameters far from satisfactory in practice. These gaps inspire us to investigate the following critical open problem: \textit{is it possible to design a systematic approach that can find SecureBoost hyperparameters to achieve optimal tradeoffs between utility, efficiency, and privacy?}

% \red{revise following by Ren}

% By adjusting the hyperparameters of the model, the privacy leakage risk of the model can be reduced at the cost of lowering the accuracy and efficiency. The optimization goals of utility, efficiency, and privacy form a trade-off, and we need to optimize these three goals simultaneously, which is also known as trustworthy federated learning. 

Our work provides a positive answer to this question. More specifically, we apply Constrained Multi-Objective Federated Learning (CMOFL)~\cite{kang2023optimizing} to find Pareto optimal solutions of hyperparameters that can minimize utility loss, training cost, and privacy leakage simultaneously. Each solution is an optimal tradeoff between the three conflicting objectives. As a result, Pareto optimal solutions not only provide optimal hyperparameters for SecureBoost but also can support the flexible requirements of FL participants. For example, FL participants can select the most appropriate hyperparameters from the Pareto optimal solutions that satisfy their current preference over utility, efficiency, and privacy.

% be employed to optimize solutions to this problem, which is designed to optimize multiple objectives in federated learning. The main challenge lies in how to choose the optimization objectives of SecureBoost reasonably and select appropriate parameters for multi-objective optimization in federated learning. 

% There are two main challenges in this multi-objective optimization problem. First, the current hyperparameter tuning methods for SecureBoost mainly use grid search and other methods, which are inefficient in the federated setting and require significant computational resources to search for a set of solutions. Second, there is no discussion on the label leakage of SecureBoost, and there is a lack of a privacy leakage measurement.

% Genetic algorithm can be used to solve the multi-objective optimization problem in federated learning\cite{DBLP:journals/tnn/ZhuJ20}, avoiding the huge computational cost issues caused by grid search and random search. 
% The calculated Pareto front can be used as guidance for hyperparameter selection in federated learning, and suitable hyperparameters can be selected according to user preferences.

% In this paper, we propose the SecureBoost hyper-parameter optimization framework that models the problem as a multi-objective optimization task. This approach offers guidance for selecting SecureBoost hyper-parameters, achieving a favorable tradeoff among efficiency, utility, and privacy. We found that there is a risk of label leakage in SecureBoost and identified a measurement to quantify the degree of privacy leakage. Additionally, we propose some methods to suppress the privacy leakage of SecureBoost. Finally, we validate through experiments that there exists a tradeoff among utility, efficiency, and privacy, and the proposed framework can find a set of solutions that are better than the default parameters.

% In this paper, we introduce three optimization objectives for SecureBoost in terms of privacy, utility, and efficiency. Our proposed CMOSB framework simultaneously optimizes these three objectives and can compute the Pareto front, providing guidance for hyperparameter selection. Finally, we validated through experiments that the Pareto solutions found by our proposed algorithm are superior to empirical hyperparameters. 

% In this paper, we propose the SecureBoost hyper-parameter optimization framework CMOSB that models the problem as a multi-objective optimization task. This approach offers guidance for selecting SecureBoost hyper-parameters, achieving a favorable tradeoff among efficiency, utility, and privacy. We found that there is a risk of label leakage in SecureBoost and identified a measurement to quantify the degree of privacy leakage. Additionally, we propose some methods to suppress the privacy leakage of SecureBoost. Finally, we validate through experiments that there exists a tradeoff among utility, efficiency, and privacy, and the proposed framework can find a set of solutions that are better than the default parameters.

Our main contributions are summarized as follows: 
% \vspace{-0.4em}
\begin{itemize}
    % \item We design the measurement for SecureBoost in terms of privacy, utility and efficiency. 
    \item We apply Constrained Multi-Objective Federated Learning (CMOFL) to SecureBoost and propose a Constrained Multi-Objective SecureBoost (CMOSB) algorithm (Sec.~\ref{sec:mosb}) to find the Pareto optimal solutions of hyperparameters that minimize utility loss, training cost, and privacy leakage simultaneously. This is one of the first attempts to apply CMOFL to VFL in general and SecureBoost in particular. 
    \item We design measurements of utility loss, training cost, and privacy leakage for SecureBoost. In particular, privacy leakage is measured by our proposed label inference attack (Sec. \ref{sec:attack}). We also develop two countermeasures against this attack (Sec.~\ref{sec:defense}).
    \item We conduct experiments on four datasets, demonstrating that our CMOSB can find better hyperparameters than grid search and Bayesian optimization in terms of the tradeoff between privacy leakage, utility loss, and training cost. Moreover, CMOSB can find Pareto optimal solutions of hyperparameters that achieve the optimal tradeoffs between utility loss, training cost, and privacy leakage (Sec.~\ref{sec:exp}).
\end{itemize}

% This paper is organized as follows. 
% Section \ref{sec:rel} introduces the related work. 
% Section \ref{sec:bac} presents the background of Secureboost and multi-objective federated learning. 
% A detailed description of the proposed framework is given in Section \ref{sec:cmosb}. 
% Section \ref{sec:exp} presents and discusses the experimental results.
% Finally, this paper is concluded in Section 6.

